Distributed Fair Scheduling for Information Exchange in Multi-Agent Systems

Information exchange is a crucial component of many real-world multi-agent systems. However, the communication between the agents involves two major challenges: the limited bandwidth, and the shared communication medium between the agents, which restricts the number of agents that can simultaneously exchange information. While both of these issues need to be addressed in practice, the impact of the latter problem on the performance of the multi-agent systems has often been neglected. This becomes even more important when the agents' information or observations have different importance, in which case the agents require different priorities for accessing the medium and sharing their information. Representing the agents' priorities by fairness weights and normalizing each agent's share by the assigned fairness weight, the goal can be expressed as equalizing the agents' normalized shares of the communication medium. To achieve this goal, we adopt a queueing theoretic approach and propose a distributed fair scheduling algorithm for providing weighted fairness in single-hop networks. Our proposed algorithm guarantees an upper-bound on the normalized share disparity among any pair of agents. This can particularly improve the short-term fairness, which is important in real-time applications. Moreover, our scheduling algorithm adjusts itself dynamically to achieve a high throughput at the same time. The simulation results validate our claims and comparisons with the existing methods show our algorithm's superiority in providing short-term fairness, while achieving a high throughput.

==> lemma_delta.tex <==
\section*{Appendix}
\subsection*{Proof of Lemma \ref{fin_servdev}}~\label{fin_servdev_proof}
\begin{proof}
Let us define $b_k^i$ as $\max\{a_k^i,d_k^{i-1}\}$. If packet $p_k^i$ arrives before that packet $p_k^{i-1}$ has finished its service, $b_k^i=d_k^{i-1}$ and hence
\begin{equation}\label{ee}
\delta_k(b_k^i)=\delta_k(d_k^{i-1}), \qquad a_k^i<d_k^{i-1} . 
\end{equation}
Otherwise, $b_k^i=a_k^i>d_k^{i-1}$ and therefore we have
\begin{equation}\label{cc}
\delta_k(b_k^i)=\delta_k(a_k^i)=\delta_k(d_k^{i-1})+\delta_k(d_k^{i-1},a_k^i)\\
\end{equation}
Since flow $k$ is not backlogged during the interval $(d_k^{i-1},a_k^i)$, we get
\begin{equation}\label{dd}
\delta_k(d_k^{i-1},a_k^i)=v(d_k^{i-1},a_k^i)-v_k(d_k^{i-1},a_k^i)=0.
\end{equation}
We conclude from (\ref{ee}), (\ref{cc}) and (\ref{dd}) that:
\begin{equation}
\delta_k(b_k^i)=\delta_k(d_k^{i-1}) \label{16}.
\end{equation}
On the other hand, according to the definition of $b_k^i$,  all the previous packets of flow $k$ have been sent by time $b_k^i$. So, $p_k^i$ is  the only packet that will be transmitted by flow $k$ during $(b_k^i,d_k^i)$. Furthermore, transmitting $p_k^i$ requires sensing the channel idle for $B_k^i$ generalized slots. Consequently, during the interval $(b_k^i,d_k^i)$, normalized service of flow $k$ and the network's virtual time will be increased by  $L_k^i/\phi_k$ and $B_k^i/\alpha$, respectively, i.e.,
\begin{align}
v_k(b_k^i,d_k^i)&=w_k(b_k^i,d_k^i)=\frac{L_k^i}{\phi_k}, \label{17}\\
v(b_k^i,d_k^i)&=\frac{B_k^i}{\alpha}=\frac{\lfloor \alpha (\frac{L_k^i}{\phi_k} - \epsilon_k^i ) \rfloor}{\alpha} \label{18}.
\end{align} 

%Considering the fact that flow $k$ is constantly backlogged during the interval $(b_k^i,d_k^i)$, we have $v_k(b_k^i,d_k^i)=w_k(b_k^i,d_k^i)$.  
Using Eqs.~(\ref{17}) and (\ref{18}), we get 
\begin{align}
\delta_k(b_k^i,d_k^i)&=v(b_k^i,d_k^i)-v_k(b_k^i,d_k^i) \\
&=\frac{\lfloor \alpha (\frac{L_k^i}{\phi_k} - \epsilon_k^i ) \rfloor}{\alpha} - \frac{L_k^i}{\phi_k} \label{21}
\end{align}

Let us return to the definition of $\epsilon_k^i$. Comparing Eqs.~(\ref{4}) and (\ref{21}) we get
\begin{align}
\epsilon_k^{i+1} - \epsilon_k^{i}&=\delta_k(b_k^i,d_k^i)  
\end{align}
Furthermore:
\begin{align}
\epsilon_k^i&=\epsilon_k^1+\sum_{n=1}^{i-1} (\epsilon_k^{n+1}-\epsilon_k^n)=\sum_{n=1}^{i-1} \delta_k(b_k^{n},d_k^n) \nonumber \\
 \nonumber \\
&= \delta_k(b_k^{1},d_k^{1})+\sum_{n=2}^{i-1} \delta_k(b_k^{n},d_k^n).
\end{align}
Using Eq.~(\ref{16}) and considering the fact that $\delta_k(b_k^1)=0$, since $b_k^1$ is the first time that flow $k$ gets backlogged and consequently $v(b_k^1)=v_k(b_k^1)$, we get the following equation:
\begin{align}
\epsilon_k^i&=\delta_k(d_k^{1})+\sum_{n=2}^{i-1} \delta_k(d_k^{n-1},d_k^n) \nonumber \\
&=\delta_k(d_k^{1})+\delta_k(d_k^{1},d_k^{i-1}) =\delta_k(d_k^{i-1})\label{e_d}
\end{align}
So, \emph{CompensationFactor} for the $i$th packet of flow $k$ is actually equal to the normalized service deviation after the transmission of packet $p_k^{i-1}$. 
Defining $\gamma= \alpha ( \frac{L_k^i}{\phi_k}-\delta_k(d_k^{i-1}) )$, $\delta_k(d_k^i)$ can be simply calculated as follows:
%Combining (\ref{d_d}), (\ref{21}) and (\ref{e_d}) we get:
\begin{align}
\delta_k(d_k^i)&=\delta_k(d_k^{i-1})+\delta_k(b_k^i,d_k^i) \nonumber \\
\delta_k(d_k^i)&=\frac{\lfloor \gamma \rfloor - \gamma}{\alpha},
\end{align}
where we have used Eq.~(\ref{16}) in the first line. Since $-1~<~\lfloor \gamma \rfloor - \gamma~\leq~0$, the proof is completed.
\end{proof}


\subsection*{Background on IEEE 802.11 DCF}
Distributed Coordination Function (DCF) in IEEE 802.11 standard, is a distributed random access scheme based on the CSMA/CA protocol. Any node~$i$ wishing to transmit a new packet, chooses a uniformly distributed random integer, $B_i$, in the interval $[0 , CW]$, where $CW$ is the contention window size and equals $CW_{min}$ for the first transmission attempt. After sensing the channel idle for a DIFS interval, the transmitter node starts a backoff interval of $B_i$ slots. Backoff counter is decremented by one after each idle slot and it is frozen during busy periods. When $B_i$ reaches zero, the transmitter node sends a Request to Send (RTS) packet for the intended destination. The destination, upon receiving the RTS, sends a Clear to Send (CTS) packet. Otherwise, if the the transmitted RTS packet collides with another RTS, the transmitter will not receive a CTS packet in response and therefore finds out that its RTS packet has been collided.  Each node~$i$ that encounters a collision, doubles $CW$ up to a maximum value $CW_{max}$ and chooses a new $B_i$ in the interval $[0,CW]$. Finally, $CW$ is reset to zero after each successful transmission. 

Now, the transmitter on receipt of the CTS, starts sending the data packet and finally the receiver acknowledges the receipt of the data packet by an Acknowledgment (ACK) packet. 


\subsection*{Implementation Details}

Here, we present some modifications based on the 802.11 protocol, which address the  potential issues caused by the unrealistic assumptions we made in our system model in Section~\ref{model}. 


Our modified algorithm uses two different IFS values,  \emph{High Priority InterFrame Spacing} (HIFS) and \emph{Low Priority InterFrame Spacing} (LIFS), for classes I and II, respectively,  which are defined as follows
\begin{align*}
\textnormal{HIFS}&=\textnormal{SIFS + 2$\sigma$},  \\
\textnormal{LIFS}&=\textnormal{SIFS + 3$\sigma$}, 
\end{align*}
where SIFS is the \emph{Short InterFrame Spacing} used in 802.11 DCF, and $\sigma$ represents the length of the time slot. By defining different IFS values as above, we can prioritize class~I agents over class~II.


Now, our algorithm can be modified as follows. Let $p_k^i$ denote the $i$th packet of agent $k$. Each node then takes the following actions:
\begin{enumerate}
\item At the time packet $p_k^i$ reaches the front of its corresponding flow, it is tagged with backoff tag $B_{k}^{i}$, calculated as follows:
\begin{equation}
B_k^i=\left\lfloor \alpha (\frac{L_k^i}{\phi_k} - \epsilon_k^i ) \right\rfloor, \label{bkoff}
\end{equation}

where $L_k^i$ and $\alpha$  are the size of packet  $p_k^i$ and scaling factor, respectively, and $\epsilon_k^i $ represents \emph{CompensationFactor}, which is defined as
\begin{equation}
\begin{array}{ll}
\epsilon_k^1 &= 0, \\ 
\epsilon_k^i  &= \epsilon_k^{i-1} + (\frac{B_k^{i-1}}{\alpha} - \frac{L_k^{i-1}}{\phi_k}). \label{4}
\end{array}
\end{equation}


\item Node $k$, $k \in \text{Class~II}$, picks a backoff interval equal to  $B_k^i$ slots after sensing the channel idle for an interval of length LIFS. 
\item Whenever a node's backoff reaches zero, it transmits an RTS packet for the intended destination and waits for a predefined amount of time (\emph{CTS timeout}) to receive a CTS packet from the destination.
\item If node $k$ receives a CTS packet from the destination before \emph{CTS timeout} ends, it starts transmitting packet $p_k^i$. Otherwise, it assumes that a collision has happened and therefore increments its collision counter by 1. 
\item Each node involved in the collision makes two modifications before retransmission. First, it picks HIFS as its interframe spacing so that it gets prior access to the channel compared to other nodes that have not experienced collision. Second, in order to avoid a guaranteed collision with other Class~I nodes, node $k \in \text{Class~I}$ chooses a uniformly distributed integer, $C_k^{q_k}$, in the interval $[(q_k-1)m+1,q_km]$, where $q_k$ is node $k$'s collision counter and $m$ is an adjustable parameter.

\item  After an idle interval of length HIFS, node $k \in \text{Class~I}$ transmits a pulse for a duration of $C_k^{q_k}$ slots and then goes to the carrier sensing mode. If it concludes that the following slot is busy, it defers its transmission and repeats step~6, without changing its  collision counter. Otherwise, it will transmit an RTS packet in the next time slot. 
\item If a collision occurs, nodes involved in the collision increase their collision counters and go to step~5.    

\item Each time a node transmits successfully, it resets its collision counter to~0 and repeats the same procedure for the next packet.       
\end{enumerate}


==> theoremproof.tex <==
\section{Proof of Theorem~\ref{THEO1}}\label{append_theorem}
\end{proof}

